Event-triggered Robust Model Predictive Control under Hard Computation Resource Constraints

Model predictive control (MPC) is capable of controlling nonlinear systems with guaranteed constraint satisfaction and stability. However, MPC requires solving optimization problems online periodically, which often exceeds the local system's computational capabilities. A potential solution is to leverage external processing, such as a central industrial server. Yet, this central computer typically serves multiple systems simultaneously, leading to significant hardware demands due to the need to solve numerous optimization problems concurrently. In this work, we tackle this challenge by developing an event-triggered model predictive control (ET-MPC) that provably stabilizes multiple nonlinear systems under disturbances while solving only optimization problems for a fixed-size subset at any given time. Unlike existing ET-MPC methods, which primarily reduce average computational load yet still require hardware capable of handling all systems simultaneously, our approach reduces the worst-case computational load. This significantly lowers central server hardware requirements by diminishing peak computational demands. We achieve our improvements by leveraging recent advancements in distributed event-triggered linear control and integrating them with a robust MPC that employs constraint tightening.

==> Makros_slides.tex <==
\makeatletter
    \newenvironment{withoutheadline}{
        \setbeamertemplate{headline}[default]
        \def\beamer@entrycode{\vspace*{-\headheight}}
    }{}
\makeatother

% ------------- Creating a new block template ----------
\makeatletter
\def\th@newblock{%
  \normalfont 
  \def\inserttheoremblockenv{exampleblock}}
\theoremstyle{newblock}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\makeatother

\makeatletter
\let\HL\hl
\renewcommand\hl{%
  \let\set@color\beamerorig@set@color
  \let\reset@color\beamerorig@reset@color
  \HL}
\makeatother

\newenvironment{greenblock}[3]{%
  \setbeamercolor{block body}{#2}
  \setbeamercolor{block title}{#3}
  \begin{block}{#1}}{\end{block}}

\tikzstyle{na} = [baseline=-.5ex]


\newcommand{\fakepar}[1]{\vspace{1mm}\noindent\textbf{#1.}}
\newcommand{\capt}[1]{\mdseries{\emph{#1}}}
\newcommand*{\matlab}{\textit{Matlab}}
\newcommand*{\simulink}{\textit{Simulink}}
\newcommand*{\purepursuit}{\textit{Pure Pursuit}}
\newcommand*{\carCup}[0]{\textit{Carolo-Cup}~}
\newcommand*{\ros}[0]{\textit{ROS2}~}
\newcommand*{\psaf}[0]{Projektseminar Autonomes Fahren~}
\newcommand*{\darpa}[0]{\textit{DARPA}~}
\newcommand*{\opencv}[1]{\textit{OpenCV}}

\newcommand*{\jt}{\textit{Jetson TX2}}
\newcommand*{\jpi}{\textit{SDK Manager}}

% Formeln
\newcommand*{\phil}{\ensuremath{\varphi_\textrm{L}}}
\newcommand*{\philmax}{\ensuremath{\varphi_\textrm{L,max}}}
\newcommand*{\dphilmax}{\ensuremath{\dot{\varphi_\textrm{L,max}}}}

% Definition für Vektor und Matizen
\newcommand*{\mat}[1]{{\ensuremath{\mathrm{\textbf{#1}}}}}
\newcommand*{\ma}[1]{{\ensuremath{\boldsymbol{\mathrm{#1}}}}}
\newcommand*{\mas}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand*{\ve}[1]{{\ensuremath{\boldsymbol{#1}}}}
\newcommand*{\ves}[1]{\ensuremath{\boldsymbol{\mathrm{#1}}}}

\newcommand*{\AP}{\ensuremath{\mathrm{AP}}}
\newcommand*{\doti}{\ensuremath{(i)^\cdot}}

\newcommand*{\inprod}[2]{\ensuremath{\langle #1,\,#2 \rangle}}

% Problem mit Siunitx
%\newcommand*{\ul}[1]{\underline{#1}}

% gerades "d" (z.B. für Integral)
\newcommand*{\ud}{\ensuremath{\mathrm{d}}}

% normaler Text in Formeln
\newcommand*{\tn}[1]{\textnormal{#1}}

% nicht-kursive Schrift in Formeln
\newcommand*{\mrm}[1]{\ensuremath{\mathrm{#1}}}

% gerades "T" für Transponiert
\newcommand*{\transp}{\ensuremath{\mathrm{T}}}

% gerades "rg"
\newcommand*{\rang}{\ensuremath{\operatorname{rg}}}

% Für geklammerte Ausdrücke mit Index (Subscript)
% (einmal mit kursiven Index, einmal mit geradem Index)
\newcommand*{\grpsb}[2]{\ensuremath{\left(#1\right)_{#2}}}
\newcommand*{\grprsb}[2]{\ensuremath{\left(#1\right)_{\mathrm{#2}}}}

% Ableitungen und Integrale
% "normale" Ableitung (mit geraden "d"s)
\newcommand*{\normd}[2]{\ensuremath{\frac{\mathrm{d}#1}{\mathrm{d}#2}}}
\newcommand*{\normdat}[3]{\ensuremath{\left.\frac{\mathrm{d} #1}{\mathrm{d} #2}\right|_{#3}}}

% Materielle Ableitung
\newcommand*{\matd}[2]{\ensuremath{\frac{\mathrm{D} #1}{\mathrm{D} #2}}}
\newcommand*{\matdat}[3]{\ensuremath{\left.\frac{\mathrm{D} #1}{\mathrm{D} #2}\right|_{#3}}}

% Partielle Ableitung
\newcommand*{\partiald}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
\newcommand*{\partialdat}[3]{\ensuremath{\left.\frac{\partial #1}{\partial #2}\right|_{#3}}}


% Transformationen
\newcommand*{\FT}[1]{\ensuremath{\mathfrak{F}\left\{#1\right\}}}
\newcommand*{\FTabs}[1]{\ensuremath{\left|\mathfrak{F}\left\{#1\right\}\right|}}
\newcommand*{\IFT}[1]{\ensuremath{\mathfrak{F}^{-1}\left\{#1\right\}}}
\newcommand*{\DFT}[1]{\ensuremath{\mathrm{DFT}\left\{#1\right\}}}
\newcommand*{\DFTabs}[1]{\ensuremath{\left|\mathrm{DFT}\left\{#1\right\}\right|}}
\newcommand*{\Laplace}[1]{\ensuremath{\mathfrak{L}\left(#1\right)}}
\newcommand*{\InvLaplace}[1]{\ensuremath{\mathfrak{L^{-1}}\left(#1\right)}}
\newcommand*{\invtrans}{\ensuremath{\quad\bullet\!\!-\!\!\!-\!\!\circ\quad}}
\newcommand*{\trans}{\ensuremath{\quad\circ\!\!-\!\!\!-\!\!\bullet\quad}}





% Manche textcomp-Zeichen funktionieren mit dem TU-Design nicht, diese können dann mit diesem
% Befehl gesetzt werden.
\newcommand*{\textcompstdfont}[1]{{\fontfamily{cmr} \fontseries{m} \fontshape{n} \selectfont #1}}

\newcommand*{\mlfct}[1]{\texttt{#1}}

\newcommand*{\UL}[2]{#1_\mathrm{#2}}
\newcommand*{\ULi}[2]{#1_{#2}}
\newcommand*{\dy}[0]{\dot{y}}
\newcommand*{\ddy}[0]{\ddot{y}}
\newcommand*{\receivedPower}[0]{\frac{A}{y^2+h^2}}
\newcommand*{\dD}[0]{\dot{D}}
\newcommand*{\tf}[0]{\UL{t}{f}}
\newcommand*{\umax}[0]{\UL{u}{max}}

\newcommand*{\x}[1]{\UL{x}{#1}}
\newcommand*{\xv}[0]{\ve{x}}
\newcommand*{\la}[1]{\UL{\lambda}{#1}}
\newcommand*{\ua}[0]{\UL{u}{+}}
\newcommand*{\ub}[0]{\UL{u}{-}}
\newcommand*{\Ht}[1]{\tilde{H}(#1)}
\newcommand*{\Dp}[0]{\UL{D}{p}}
\newcommand*{\Dm}[0]{\overline{\dot{D}}}
\newcommand*{\fdynamic}[0]{\UL{\ve{f}}{dynamic}(\ve{y}, u)}
\newcommand*{\fE}[0]{\UL{f}{E}(\ve{y}, u)}
\newcommand*{\fD}[0]{\UL{f}{D}(\ve{y}, u)}
\newcommand*{\vl}[0]{\UL{v}{l}}
\newcommand{\vex}[0]{\ve{x}}
\newcommand*{\of}[1]{(#1)}
%\renewcommand*{\of}[1]{{}_{,#1}}
\newcommand*{\vexof}[1]{\vex\of{#1}}
\newcommand*{\vexul}[1]{\UL{\vex}{#1}}
\newcommand*{\vexulof}[2]{\UL{\vex}{#1}\of{#2}}
\newcommand*{\vexuli}[1]{\ULi{\vex}{#1}}
\newcommand*{\hatvexuli}[1]{\ULi{\hat{\vex}}{#1}}
\newcommand*{\vexuliof}[2]{\ULi{\vex}{#1}\of{#2}}
\newcommand*{\hatvexuliof}[2]{\ULi{\hat{\vex}}{#1}\of{#2}}
\newcommand*{\pcom}[0]{{P\ul{com}}}
\newcommand*{\pcomhat}[0]{\hat{P}\ul{com}{}}
\newcommand{\weight}[2]{w\uliof{#1}{#2}}
\newcommand{\history}[0]{\mathcal{E}}
\newcommand{\weighthat}[2]{\hat{w}\uliof{#1}{#2}}

\newcommand*{\veerr}[0]{\ve{e}}
\renewcommand*{\ul}[1]{_{\mathrm{#1}} }
\newcommand*{\uliof}[2]{_{#1}{\of{#2}}}
\newcommand*{\uli}[1]{_{#1} }
\newcommand*{\koop}[0]{\mathcal{K}}
\newcommand*{\koopt}[0]{\mathcal{K}^t}
\newcommand*{\gof}[1]{g\of{#1}}
\newcommand*{\gul}[1]{\ULi{g}{#1}}
\newcommand*{\gofxof}[1]{\gof{\vexof{#1}}}
\newcommand*{\phivexof}[1]{\phi\of{\vexof{#1}}}
\newcommand*{\veg}[0]{\ve{g}}
\newcommand*{\vegof}[1]{\ve{g}\of{#1}}
\newcommand*{\vegulof}[2]{\ve{g}_{\mathrm{#1}}\of{#2}}
\newcommand*{\vey}[0]{\ve{y}}
\newcommand*{\veyof}[1]{\vey\of{#1}}
\newcommand*{\veyul}[1]{\UL{\vey}{#1}}
\newcommand*{\tzero}[0]{\UL{t}{0}}
\newcommand*{\vepsi}[0]{\ve{\psi}}
\newcommand*{\vephi}[0]{\ve{\phi}}
\newcommand*{\veu}[0]{\ve{u}}
\newcommand*{\veuof}[1]{\veu\of{#1}}
\newcommand*{\veuul}[1]{\UL{\veu}{#1}}
\newcommand*{\vev}[0]{\ve{v}}
\newcommand*{\vevof}[1]{\vev\of{#1}}
\newcommand*{\vevul}[1]{\UL{\vev}{#1}}
\newcommand*{\xul}[1]{\ULi{x}{#1}}
\newcommand*{\aul}[1]{\UL{a}{#1}}
%\newcommand*{\bul}[1]{\UL{b}{#1}}
\newcommand*{\kul}[1]{\UL{k}{#1}}
\newcommand*{\uul}[1]{\ULi{u}{#1}}

\newcommand*{\maAuli}[1]{\ULi{\ma{A}}{#1}}
\newcommand*{\veeps}[0]{\ve{\epsilon}}
\newcommand*{\twonorm}[1]{||#1||_\mathrm{2}}

\newcommand*{\lambdamaxof}[1]{\UL{\lambda}{max}\of{#1}}
\newcommand*{\lambdaminof}[1]{\UL{\lambda}{min}\of{#1}}
% Problem mit Siunitx
%\newcommand*{\A}[0]{Method A\:}
\newcommand*{\B}[0]{Method B\:}
%\newtheorem{definition}{Definition}[section]

%\newcommand*{\q}{q_\ve{\theta}}

%\newcommand*{\g}[1]{g\uli{#1}}
%\newcommand*{\e}[2]{%
%\ifthenelse { \equal {#2} {} }  %if short caption not specified, use long caption (no slant)
%{ \veerr\uli{#1} }   % if #2 == blank
%{ \veerr\uli{#1}\of{#2} }   % else (not blank)

%}

\newcommand*{\matA}[1]{\ma{A}\uli{#1}}
\newcommand*{\matGamma}[0]{\ma{\Gamma}}
\newcommand*{\matGammaOpt}[0]{\ma{\Gamma}\ul{opt}}

\newcommand*{\matQ}[1]{{\ma{Q}\uli{#1}}}
\newcommand*{\matP}[1]{\ma{P}\uli{#1}}
\newcommand*{\eps}[2]{\epsilon\uli{#1}\of{#2}}
\newcommand*{\alp}[2]{\alpha\uli{#1}\of{#2}}
\newcommand*{\pfail}[0]{P\ul{loss}}
\newcommand{\priority}[2]{g\uli{#1}\of{\errorest{#1#1}{#2}}}
\newcommand*{\diag}[0]{\text{diag}}
\newcommand*{\tp}[1]{\of{#1}}
\newcommand*{\state}[2]{\vex\uli{#1}\tp{#2}}
\newcommand*{\stateest}[2]{\hat{\vex}\uli{#1}\tp{#2}}
\newcommand*{\noise}[2]{\ve{w}\uli{#1}\tp{#2}}
\newcommand*{\processnoise}[2]{\ve{v}\uli{#1}\tp{#2}}
\newcommand*{\errart}[2]{\ve{\tilde{e}}\uli{#1}\tp{#2}}
\newcommand*{\errorest}[2]{\ve{e}\uli{#1}\tp{#2}}
\newcommand*{\barerrorest}[2]{\ve{\bar{e}}\uli{#1}\tp{#2}}
\newcommand*{\errorestmeas}[2]{\ve{e}\uli{#1, meas}\tp{#2}}
\newcommand*{\erroragents}[2]{\hat{\ve{e}}\uli{#1}\tp{#2}}
\newcommand*{\erroragentstotal}[2]{\underline{\hat{\ve{e}}}\uli{#1}\tp{#2}}
\newcommand*{\erroresttotal}[2]{\underline{\ve{e}}\uliof{#1}{#2}}
\newcommand*{\matB}[1]{\ma{B}\uli{#1}}
\newcommand*{\matV}[1]{\ma{V}\uli{#1}}
\newcommand*{\matVti}[1]{\ma{\tilde{V}}\uli{#1}}
\newcommand*{\matW}[1]{\ma{W}\uli{#1}}
\newcommand*{\matAT}[1]{\left(\ma{A}\uli{#1}^\transp\right)}
\newcommand*{\matF}[1]{\ma{F}\uli{#1}}
\newcommand*{\rec}[2]{\gamma\uli{#1}\tp{#2}}
\newcommand*{\Cov}{\mathrm{Cov}}
\newcommand*{\matAti}[1]{\tilde{\ma{A}}\uli{#1}}

\newcommand{\io}[1]{\Gamma\of{#1}}
\newcommand{\oi}[1]{\Lambda\of{#1}}

\newcommand{\matAd}[1]{\tilde{\mat{A}}\ul{d, \mathrm{#1}}}
\newcommand{\ri}[1]{{r\uli{#1}}}
\newcommand{\di}[1]{{d\uli{#1}}}
\newcommand{\nii}[1]{{n\uli{#1}}}
\newcommand{\deltai}[1]{\Delta\uli{#1}}
\newcommand{\betai}[1]{\beta\uli{#1}}
\newcommand{\alphai}[1]{\alpha\uli{#1}}
\newcommand{\zetai}[1]{\zeta\uli{#1}}
\newcommand{\lmax}[1]{\lambda\ul{max}\of{#1}}
\newcommand{\lmin}[1]{\lambda\ul{min}\of{#1}}
\newcommand{\unknown}[0]{\left(\cdot\right)}
\newcommand*{\kt}[0]{\tilde{k}}
\newcommand*{\nz}[0]{\ve{n}\ul{0}}
\newcommand*{\norm}[2]{||#1||_{#2}}
\newcommand*{\diff}[0]{\text{d}}

\newcommand{\dalpha}[0]{\delta\alpha}
\newcommand{\setS}[0]{\mathcal{S}}
\newcommand{\cone}[0]{c\ul{1}\of{\setS}}
\newcommand{\ctwo}[0]{c\ul{2}\of{\setS}}

\newcommand{\pos}[0]{\ve{p}}
\newcommand{\speed}[0]{\ve{v}}
\newcommand{\acc}[0]{\ve{a}}

\newcommand{\posset}[1]{\pos\uli{#1, \mathrm{set}}}
\newcommand{\speedset}[1]{\speed\uli{#1, \mathrm{set}}}
\newcommand{\accset}[1]{\acc\uli{#1, \mathrm{set}}}
\newcommand{\vexset}[1]{\vex\uli{#1, \mathrm{set}}}
\renewcommand{\posset}[1]{\pos\uli{#1}}
\renewcommand{\speedset}[1]{\speed\uli{#1}}
\renewcommand{\accset}[1]{\acc\uli{#1}}
\renewcommand{\vexset}[1]{\vex\uli{#1}}
\newcommand{\stimeobj}[0]{T\ul{o}}
\newcommand{\stimes}[0]{T\ul{s}}
\newcommand{\stimecons}[0]{T\ul{b}}
\newcommand{\stimecol}[0]{T\ul{c}}
\newcommand{\dxmax}[2]{\Delta\vexset{#1}{}\ul{max}\of{#2}}
\newcommand{\dpmax}[2]{\Delta\posset{#1}{}\ul{,max}\of{#2}}

\newcommand{\cu}{CU}
\newcommand{\cus}{CUs}
\newcommand{\artinput}{\ve{u}}
\newcommand{\artinputset}{\mathcal{u}}

\newcommand{\gp}[2]{\mathcal{GP}\of{#1, #2}}
\newcommand{\kernel}[3]{k\ul{#1}\of{#2, #3}}
\newcommand{\tkernel}[2]{\kernel{t}{#1}{#2}}
\newcommand{\xkernel}[2]{\kernel{x}{#1}{#2}}
\newcommand{\mkernel}[3]{K\ul{#1}\of{#2, #3}}
\newcommand{\tmkernel}[2]{\mkernel{t}{#1}{#2}}
\newcommand{\xmkernel}[2]{\mkernel{x}{#1}{#2}}
\newcommand{\realnmbrs}{\mathbb{R}}

\newcommand{\tobjfunc}[3]{J\ul{#1}\of{[#2, #3]}}
\newcommand{\tobjfuncn}[3]{\tilde{J}\ul{#1}\of{[#2, #3]}}

\newcommand{\opttheta}[2]{\theta^*\uli{#1}\of{#2}}

\newcommand{\jmin}{J_\mathrm{min}}
\newcommand{\sx}{\sigma_\mathrm{x}}
% \newcommand{\st}{\sigma_\mathrm{t}}

\newcommand{\taua}{\tau_\mathrm{a}}
\newcommand{\taub}{\tau_\mathrm{b}}

\newcommand{\xpredi}[3]{x_{#1}(#2|#3)}
\newcommand{\xpred}[2]{x(#1|#2)}
\newcommand{\xreali}[2]{x_{#1}(#2)}
\newcommand{\xreal}[1]{x(#1)}
\newcommand{\xpredopt}[2]{x^*(#1|#2)}
\newcommand{\xpredcand}[2]{\tilde{x}(#1|#2)}

%\newcommand{\dxpred}[3]{\Delta \xpredi{#1}{#2}{#3}}
\newcommand{\wart}[2]{w_\mathrm{art}(#1|#2)}
%\newcommand{\dupred}[3]{\Delta \upredi{#1}{#2}{#3}}

\newcommand{\upredi}[3]{u_{#1}(#2|#3)}
\newcommand{\upred}[2]{u(#1|#2)}
\newcommand{\ureali}[2]{u_{#1}(#2)}
\newcommand{\ureal}[1]{u(#1)}
\newcommand{\upredopt}[2]{u^*(#1|#2)}
\newcommand{\upredcand}[2]{\tilde{u}(#1|#2)}

\newcommand{\lf}[0]{L_\mathrm{f}}
\newcommand{\tc}[0]{t_\mathrm{c}}
\newcommand{\tcn}[1]{t_\mathrm{#1}}

\newcommand{\vdelta}[0]{V_\mathrm{\delta}}

\newcommand{\cdl}[0]{c_\mathrm{\delta,\ell}}
\newcommand{\cdu}[0]{c_\mathrm{\delta,u}}
\newcommand{\deltaloc}[0]{\delta_\mathrm{loc}}
\newcommand{\kmax}[0]{k_\mathrm{max}}

\newcommand{\vf}[0]{V_\mathrm{f}}
\newcommand{\vw}[0]{\tilde{V}}
\newcommand{\vwmax}[0]{\tilde{V}_\mathrm{max}}

\newcommand{\xf}[0]{\mathcal{X}_\mathrm{f}}
\newcommand{\kappaf}[0]{\kappa_\mathrm{f}}

\newcommand{\rmq}[0]{\mathrm{Q}}
\newcommand{\rmr}[0]{\mathrm{R}}
\newcommand{\rmp}[0]{\mathrm{P}}
\newcommand{\vmax}[0]{V_\mathrm{max}}



==> mainmatter/basic.tex <==

\begin{withoutheadline}
\begin{frame}{Itemize with two columns \phantom{p} \hfill \phantom{\subheadline{Subsection}}}
\begin{columns}[T]
    \column{0.45\textwidth}
        \textbf{Currently}
        \small

        \begin{itemize} % for appearing [<+-| alert@+>]
            \item Some points\\
            $\rightarrow$ follows point 1 \\
            $\rightarrow$ follows from point 1 with reference \footnotemark
            \item Some other \structure{important} points\\
            $\rightarrow$ point 3 \\
            \phantom{$\rightarrow$} linebreak
        \end{itemize}
        % \pause

        \vfill
        \centering
        \tikz[baseline]{
        \node[fill=RWTHBlue!10,rounded corners=2pt,align=left]
        {\structure{\textbf{multi-line}} \\ \structure{\textbf{conclusion}}};}

    \column{0.45\textwidth}
    % \pause
    \textbf{Some other points}
    \small
    
    \begin{itemize} % for appearing [<+-| alert@+>]
        \item other point 1 with different citation \parencite{Agrell_2019}
        \item other point 2
        \begin{itemize} % for appearing [<+-| alert@+>]
            \item with subpoints
        \end{itemize}
    \end{itemize}
    
    \end{columns}
    \footnotetext{\fullcite{Marco_2016}}
\end{frame}
\end{withoutheadline}


\begin{withoutheadline}
\begin{frame}[t]{Blocks \phantom{p} \hfill \subheadline{Subsection}}

    \begin{block}{Some block with highlighted text}
    Highlighting text can be super useful, \eg like \structure{this} or \alert{this}. However, you should not use it too often.
    It can be useful for in equations to guide the audience:
    \begin{equation}
        y(\tikz[baseline]{\node[fill=RWTHRed25,rounded corners=2pt,anchor=base] (t3)
            {$\mathbf{x}_t$};})
            =
            f_t(\tikz[baseline]{\node[fill=RWTHRed25,rounded corners=2pt,anchor=base] (t3)
            {$\mathbf{x}_t$};})
            +
            \tikz[baseline]{
            \node[fill=RWTHGreen!25,rounded corners=2pt,anchor=base] (t3)
            {$\epsilon$};}
    \end{equation}
            with 
            \tikz[baseline]{
            \node[fill=RWTHRed25,rounded corners=2pt,anchor=base] (t3)
            {query $\mathbf{x}_t$};}
            and Gaussian noise
            \tikz[baseline]{\node[fill=RWTHGreen!25,rounded corners=2pt,anchor=base] (t3){$\epsilon \sim \mathcal{N}(0, \sigma^2)$};}.
    \end{block}
    The block looks similar to:
    \begin{definition}[Some definition]
    $\mathbf{X} = \{X_1, X_2,\dots \}$
    \end{definition}
    
\end{frame}
\end{withoutheadline}

\begin{withoutheadline}
\begin{frame}[t]{More Blocks (Multi-Column) \phantom{p} \hfill \subheadline{Subsection}}

    \begin{block}{Multi-Column block}
    \dots with some interesting important stuff.
    \end{block}
    
    \begin{columns}[T]
        \column{0.47\textwidth}
        
        \begin{theorem}[Pythagorean Theorem]
        $a^2 + b^2 = c^2$.
        \end{theorem}
        
        \begin{proof}
        See: \url{https://en.wikipedia.org/wiki/Pythagorean_theorem}
        \end{proof}
        
        Column width: \the\columnwidth
        
        \column{0.47\textwidth}
        \begin{corollary}
        $a^2 + b^2 = c^2$
        \end{corollary}
        
        \begin{example}
        $2^2+2^2 = 8$.
        \end{example}
        
        \begin{alertblock}{But Careful!}
            Only right triangle!
        \end{alertblock}
    \end{columns}
\end{frame}
\end{withoutheadline}

\begin{withoutheadline}
    \begin{frame}[t]{Example Algorithm \hfill \subheadline{Subsection}}

        \textbf{TVBO Algorithm}
        \vspace{0.1cm}
        \only<1>{\begin{algorithm}[H]
        \begin{algorithmic}[1]
        \STATE GP prior $\mathcal{GP}(\mathbf{0}, k_S(\mathbf{x},\mathbf{x}') \cdot\tikz[baseline]{
                    \node[fill=white,rounded corners=2pt,anchor=base] (n1)
                    {$k_T(t, t')$};})$
        \STATE Feasible set $\mathcal{X} \in {\rm I\!R}^D$
        \STATE Data set $\mathcal{D}_{N} = \{y_j, \mathbf{x}_j, t_j\}_{j=0}^{N}$, $t_0=N$ \phantom{\qquad\qquad \tikz[baseline]{
                    \node[fill=RWTHOrange!50,rounded corners=2pt,anchor=base] (t4)
                    {C-TVBO \cmark / \xmark};}}
        \FOR{$t = t_0, t_0+1, t_0+2, \dots$ to $T$}
        \STATE Train GP model with $\mathcal{D}_t$
        \STATE Get $\hat{\mathbf{x}}^*_t = \underset{\mathbf{x}\in \mathcal{X}}{\argmin} \, \mu_{t}(\mathbf{x})$
        \STATE Optimize acquisition function $\mathbf{x}_{t+1} = \underset{\mathbf{x}\in \tilde{\mathcal{X}}_t}{\argmin} \underbrace{\tikz[baseline]{
                    \node[fill=white,rounded corners=2pt,anchor=base] (t1)
                    {$\mu_{t+1}(\mathbf{x})$};} - \tikz[baseline]{
                    \node[fill=white,opacity=0.7,rounded corners=2pt,anchor=base] (t3)
                    {$\beta $};}\tikz[baseline]{
                    \node[fill=white,rounded corners=2pt,anchor=base] (t2)
                    {$\sigma_{t+1}(\mathbf{x})$};}}_{\coloneqq \alpha_{LCB}}$
        \STATE Query objective function $y_{t+1} = f_{t+1}(\mathbf{x}_{t+1}) + w$
        \STATE $\mathcal{D}_{t+1} = \mathcal{D}_{t} \cup \{y_{t+1}, \mathbf{x}_{t+1}, t+1\}$ and data selection
        \ENDFOR
        \end{algorithmic}
        \end{algorithm}}

        \only<2>{\begin{algorithm}[H]
        \begin{algorithmic}[1]
        \STATE GP prior $\mathcal{GP}(\mathbf{0}, k_S(\mathbf{x},\mathbf{x}') \cdot\tikz[baseline]{
                    \node[fill=RWTHBlue!10,rounded corners=2pt,anchor=base] (n1)
                    {$k_T(t, t')$};})$ \qquad \tikz[baseline]{
                    \node[fill=RWTHBlue!10,rounded corners=2pt,anchor=base] (n2)
                   {\structure{\textbf{Highlight something}}};}
        \STATE Feasible set $\mathcal{X} \in {\rm I\!R}^D$
        \STATE Data set $\mathcal{D}_{N} = \{y_j, \mathbf{x}_j, t_j\}_{j=0}^{N}$, $t_0=N$ \qquad\qquad \tikz[baseline]{
                    \node[fill=RWTHOrange!50,rounded corners=2pt,anchor=base] (t4)
                    {Use it? \cmark / \xmark};}
        \FOR{$t = t_0, t_0+1, t_0+2, \dots$ to $T$}
        \STATE Train GP model with $\mathcal{D}_t$
        \STATE Get $\hat{\mathbf{x}}^*_t = \underset{\mathbf{x}\in \mathcal{X}}{\argmin} \, \mu_{t}(\mathbf{x})$
        \STATE Optimize acquisition function $\mathbf{x}_{t+1} = \underset{\mathbf{x}\in \tilde{\mathcal{X}}_t}{\argmin} \underbrace{\tikz[baseline]{
                    \node[fill=RWTHOrange!50,rounded corners=2pt,anchor=base] (t1)
                    {$\mu_{t+1}(\mathbf{x})$};} - \tikz[baseline]{
                    \node[fill=RWTHRed25,opacity=0.7,rounded corners=2pt,anchor=base] (t3)
                    {$\beta $};}\tikz[baseline]{
                    \node[fill=RWTHOrange!50,rounded corners=2pt,anchor=base] (t2)
                    {$\sigma_{t+1}(\mathbf{x})$};}}_{\coloneqq \alpha_{LCB}}$
        \STATE Query objective function $y_{t+1} = f_{t+1}(\mathbf{x}_{t+1}) + w$
        \STATE $\mathcal{D}_{t+1} = \mathcal{D}_{t} \cup \{y_{t+1}, \mathbf{x}_{t+1}, t+1\}$ and data selection
        \ENDFOR
        \end{algorithmic}
        \end{algorithm}}

        \begin{tikzpicture}[overlay]
            \path[->]<2-> (n2.north west) edge [out=160, in=40] (n1.north east);
            \path[->]<2-> (t4.south) edge [out=-90, in=90] (t1.north);
            \path[->]<2-> (t4.south) edge [out=-90, in=90] (t2.north);
        \end{tikzpicture}
    \end{frame}

\end{withoutheadline}

==> mainmatter/illustrations.tex <==


\begin{withoutheadline}
\begin{frame}[t]{Figures with .pgf \hfill \subheadline{Subsection}}
\begin{itemize}
\item Use pgf-backend from \swname{matplotlib} to have very nice figures
\end{itemize}
	\centering
	\only<1->{\input{figures/result.pgf}}
\end{frame}
\end{withoutheadline}

\begin{withoutheadline}
\begin{frame}[t]
\frametitle{Embed .gifs using .pngs \hfill \subheadline{Subsection}}
\centering	
	Uncomment in the corresponding line below \alert{(only playable in Adobe Reader!)}
	
	% COMMENT FOR VIDEO/GIF
	\begin{figure}
	    \centering
	    \includegraphics{figures/movies/example_movie/different_priors_01}
	    \caption{.png}
	    \label{fig:my_label}
	\end{figure}
	% UNCOMMENT FOR VIDEO/GIF
    % \animategraphics[controls]{4}{figures/movies/example_movie/different_priors_}{01}{10}
\end{frame}
\end{withoutheadline}

\begin{withoutheadline}
\begin{frame}[t]
\frametitle{You can use .pdf\_tex for figures  \hfill \subheadline{Subsection}}
(create them \eg with \url{https://inkscape.org/de/})
\vspace{0.5cm}
	\begin{columns}
	\column{0.45\textwidth}
	\centering
	\textbf{Sliding Window}
	\vspace{0.5cm}
	\centering
	\onslide<1->{\import{figures/}{sliding_window.pdf_tex}}
	
	\column{0.45\textwidth}	
	\centering
	\textbf{Binning}
	\vspace{0.5cm}
	\centering
	\onslide<1->{\import{figures/}{binning.pdf_tex}}
	\end{columns}
\end{frame}
\end{withoutheadline}

\begin{withoutheadline}
\begin{frame}[t]
\frametitle{Sequence of .pgf figures \hfill \subheadline{Subsection}}
    \begin{columns}[T]
    \column{0.4\textwidth}
    \begin{definition}[Some definition]
    \centering
    $\mathbf{X} \coloneqq \{X_0, X_1,\dots\}$
    \end{definition}
    
    We can also include a reference\footnote[frame]{\fullcite{Vaerenbergh_2012}}
    \begin{equation*}
        k_{T,tv}(t,t') = (1-\epsilon)^{\frac{|t-t'|}{2}}
    \end{equation*}
    and an equation :)
    
    \column{0.55\textwidth}
    \only<1>{\input{figures/b2p_forgetting.pgf}}
    
    \only<2>{\input{figures/b2p_forgetting_SE.pgf}}
    \end{columns}
    \centering
%   \vfill
    \onslide<2->{$\rightarrow$ \textbf{\structure{Note, that the figure does not jump!}}}
\end{frame}
\end{withoutheadline}

==> preamble.tex <==

%Packages for Layout
\usepackage{tikz}
\usepackage[11pt]{moresize}
\usepackage{color}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{eso-pic}
\usepackage{animate}
\usepackage{import}
\usepackage{soul}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{algorithm2e}
\usepackage{algorithmic}
\usepackage{float}

\usepackage{nccmath}

\usepackage{amssymb}    % erweiterter Zeichensatz
\usepackage{mathtools}  % erweiterte Fassung von amsmath
%\usepackage{biblatex} %Imports biblatex package
\usepackage{pgfplots}
\usepackage{tikz}
%\usepgfplotslibrary{external}
\usetikzlibrary{shapes}
\usetikzlibrary{positioning}
\usetikzlibrary{arrows,decorations.markings}
%\tikzexternalize[prefix=tikz/]
\usepackage{bm}

\usepackage{caption}
\usepackage{subcaption}
\usepackage{siunitx}

\usepackage{pgfplots}
\pgfplotsset{compat=1.18}
\usepackage{tikz}
\usepackage{hyperref}
%\usepgfplotslibrary{external}
\usetikzlibrary{positioning}
\usetikzlibrary{arrows,decorations.markings}
\usetikzlibrary{spy}

\newtheorem{assumption}{Assumption}
\newtheorem{eventtrigger}{Event-Trigger}
\newtheorem{remark}{Remark}

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\textcolor{green!50!black}{\ding{51}}}%
\newcommand{\xmark}{\textcolor{RWTHRed}{\ding{55}}}%

\renewcommand{\algorithmicrequire}{\textbf{Initialize:}} 
\renewcommand{\algorithmicensure}{\textbf{Output:}} 
\DeclareMathOperator*{\argmin}{arg\,min}

% \usepackage{times}
\usepackage{verbatim}
\usetikzlibrary{arrows,shapes}
\usetikzlibrary{tikzmark,fit}

\usefonttheme[onlymath]{serif}

%\usepackage{amsfonts, amsmath, amssymb}

\newcommand{\swname}[1]{\texttt{#1}}
\newcommand{\ie}{i\/.\/e\/.,\/~}
\newcommand{\eg}{e\/.\/g\/.,\/~}
\newcommand{\cf}{cf\/.\/~}

\newcommand{\fig}{Fig\/.\/~}
\newcommand{\defn}{Def\/.\/~}
\newcommand{\sect}{Sec\/.\/~}
\newcommand{\tabl}{Tab\/.\/~}
\newcommand{\algo}{Algorithm~}
\newcommand{\theo}{Theorem~}

\newcommand{\R}{\mathrm{I\!R}}
\newcommand{\argmax}{\arg\max} 
\DeclareMathOperator{\EX}{\mathbb{E}}
